Conf-Guard: Dynamic Multi-Turn Jailbreak Detection with Conformal Guarantees

As the applications of large language models (LLMs) expand to critical domains, their capacity for abstention becomes increasingly vital. Current methods treat abstention mostly as a single-turn problem, rather than a conversational one. This issue is of particular importance for securing LLMs against adversarial threats, which have recently shifted from single-turn attacks to sophisticated conversational exploits where malicious intent gradually unfolds across multiple turns. Traditional defences struggle to guard against multi-turn attacks and do not offer formal guarantees on the percentage of attacks they block. Here, we propose Conf-Guard, a novel framework that operates by keeping track of a scalar score which dynamically evolves throughout the conversation, and by terminating the conversation if the score breaches a threshold. We show that the threshold can be selected so as to achieve a distribution-free conformal guarantee, which, for jailbreak detection, formally ensures a user-specified percentage of attacks is successfully blocked. We also propose specific choices of score functions obtained by combining leading pre-trained jailbreak detection classifiers with an outlier detection metric. Through extensive empirical experiments, we show that Conf-Guard achieves its conformal guarantee and that our proposed score functions result in improved false refusal rates over their underlying classifiers. Our code is available at https://github.com/layer6ai-labs/conf_guard. Warning: the data we use in this paper contains jailbreak attacks with toxic and offensive language.

==> tables/turn_level_ft_overall_results.tex <==
\begingroup
\centering
\scriptsize
\setlength{\tabcolsep}{1.35pt}
\renewcommand{\arraystretch}{1.08}
\setlength{\LTleft}{0pt plus 1fill}
\setlength{\LTright}{0pt plus 1fill}

\begin{longtable}{@{}
>{\raggedright\arraybackslash}p{1.35cm}
l
*{8}{r}
@{}}
\caption{Performances at different FRR for fine-tuned LPG-2 in turn-level. All experiments use the prompt-only setting. LPG-2-FT denotes LlamaPromptGuard-2-86M fine-tuned and LPG2-FT-Cal30 denotes its calibration 30\% variant.}
\label{tab:lpg2_ft_asr}\\
\toprule
\textbf{Dataset} &
\textbf{Method} &
\textbf{ASR@1\%} &
\textbf{ASR@5\%} &
\textbf{ASR@10\%} &
\textbf{ASR@15\%} &
\textbf{ASR$_P$@1\%} &
\textbf{ASR$_P$@5\%} &
\textbf{ASR$_P$@10\%} &
\textbf{ASR$_P$@15\%} \\
\midrule
\endfirsthead

\multicolumn{10}{c}{\tablename~\thetable{} -- continued from previous page} \\
\toprule
\textbf{Dataset} &
\textbf{Method} &
\textbf{ASR@1\%} &
\textbf{ASR@5\%} &
\textbf{ASR@10\%} &
\textbf{ASR@15\%} &
\textbf{ASR$_P$@1\%} &
\textbf{ASR$_P$@5\%} &
\textbf{ASR$_P$@10\%} &
\textbf{ASR$_P$@15\%} \\
\midrule
\endhead

\midrule
\multicolumn{10}{r}{Continued on next page} \\
\endfoot

\bottomrule
\endlastfoot

\multicolumn{10}{@{}l}{\textbf{Classifier: LlamaPG-2-FT}} \\*
\midrule
\multirow{2}{=}{SA-WC-HC}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{88.76\%\\ {$\scriptsize \pm6.70\%$}} & \shortstack[r]{73.03\%\\ {$\scriptsize \pm9.41\%$}} & \shortstack[r]{71.91\%\\ {$\scriptsize \pm9.53\%$}} & \shortstack[r]{64.04\%\\ {$\scriptsize \pm10.17\%$}}
& \shortstack[r]{88.76\%\\ {$\scriptsize \pm6.70\%$}} & \shortstack[r]{73.03\%\\ {$\scriptsize \pm9.41\%$}} & \shortstack[r]{71.91\%\\ {$\scriptsize \pm9.53\%$}} & \shortstack[r]{64.04\%\\ {$\scriptsize \pm10.17\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{100.00\%\\ {$\scriptsize \pm0.00\%$}} & \shortstack[r]{97.75\%\\ {$\scriptsize \pm3.14\%$}} & \shortstack[r]{95.51\%\\ {$\scriptsize \pm4.39\%$}} & \shortstack[r]{95.51\%\\ {$\scriptsize \pm4.39\%$}}
& \shortstack[r]{100.00\%\\ {$\scriptsize \pm0.00\%$}} & \shortstack[r]{97.75\%\\ {$\scriptsize \pm3.14\%$}} & \shortstack[r]{95.51\%\\ {$\scriptsize \pm4.39\%$}} & \shortstack[r]{95.51\%\\ {$\scriptsize \pm4.39\%$}} \\
\midrule

\multirow{2}{=}{Gemini-HC}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{58.65\%\\ {$\scriptsize \pm6.83\%$}} & \shortstack[r]{38.94\%\\ {$\scriptsize \pm6.76\%$}} & \shortstack[r]{27.40\%\\ {$\scriptsize \pm6.19\%$}} & \shortstack[r]{14.90\%\\ {$\scriptsize \pm4.94\%$}}
& \shortstack[r]{59.13\%\\ {$\scriptsize \pm6.82\%$}} & \shortstack[r]{39.90\%\\ {$\scriptsize \pm6.79\%$}} & \shortstack[r]{27.40\%\\ {$\scriptsize \pm6.19\%$}} & \shortstack[r]{14.90\%\\ {$\scriptsize \pm4.94\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{95.19\%\\ {$\scriptsize \pm2.97\%$}} & \shortstack[r]{87.98\%\\ {$\scriptsize \pm4.51\%$}} & \shortstack[r]{77.88\%\\ {$\scriptsize \pm5.76\%$}} & \shortstack[r]{74.52\%\\ {$\scriptsize \pm6.04\%$}}
& \shortstack[r]{95.67\%\\ {$\scriptsize \pm2.82\%$}} & \shortstack[r]{88.94\%\\ {$\scriptsize \pm4.35\%$}} & \shortstack[r]{78.37\%\\ {$\scriptsize \pm5.71\%$}} & \shortstack[r]{75.00\%\\ {$\scriptsize \pm6.00\%$}} \\
\midrule

\multirow{2}{=}{GPT-HC}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{22.60\%\\ {$\scriptsize \pm5.80\%$}} & \shortstack[r]{13.94\%\\ {$\scriptsize \pm4.80\%$}} & \shortstack[r]{8.17\%\\ {$\scriptsize \pm3.80\%$}} & \shortstack[r]{4.81\%\\ {$\scriptsize \pm2.97\%$}}
& \shortstack[r]{40.87\%\\ {$\scriptsize \pm6.82\%$}} & \shortstack[r]{23.56\%\\ {$\scriptsize \pm5.88\%$}} & \shortstack[r]{12.50\%\\ {$\scriptsize \pm4.59\%$}} & \shortstack[r]{6.25\%\\ {$\scriptsize \pm3.36\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{62.98\%\\ {$\scriptsize \pm6.70\%$}} & \shortstack[r]{47.12\%\\ {$\scriptsize \pm6.92\%$}} & \shortstack[r]{39.90\%\\ {$\scriptsize \pm6.79\%$}} & \shortstack[r]{37.50\%\\ {$\scriptsize \pm6.71\%$}}
& \shortstack[r]{96.15\%\\ {$\scriptsize \pm2.67\%$}} & \shortstack[r]{78.37\%\\ {$\scriptsize \pm5.71\%$}} & \shortstack[r]{68.75\%\\ {$\scriptsize \pm6.43\%$}} & \shortstack[r]{62.98\%\\ {$\scriptsize \pm6.70\%$}} \\
\midrule

\multirow{2}{=}{\shortstack[l]{Gemini}}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{51.92\%\\ {$\scriptsize \pm6.93\%$}} & \shortstack[r]{35.10\%\\ {$\scriptsize \pm6.62\%$}} & \shortstack[r]{23.56\%\\ {$\scriptsize \pm5.88\%$}} & \shortstack[r]{14.42\%\\ {$\scriptsize \pm4.87\%$}}
& \shortstack[r]{64.90\%\\ {$\scriptsize \pm6.62\%$}} & \shortstack[r]{44.71\%\\ {$\scriptsize \pm6.89\%$}} & \shortstack[r]{30.77\%\\ {$\scriptsize \pm6.40\%$}} & \shortstack[r]{19.71\%\\ {$\scriptsize \pm5.52\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{72.60\%\\ {$\scriptsize \pm6.19\%$}} & \shortstack[r]{59.13\%\\ {$\scriptsize \pm6.82\%$}} & \shortstack[r]{48.08\%\\ {$\scriptsize \pm6.93\%$}} & \shortstack[r]{37.02\%\\ {$\scriptsize \pm6.70\%$}}
& \shortstack[r]{87.50\%\\ {$\scriptsize \pm4.59\%$}} & \shortstack[r]{72.60\%\\ {$\scriptsize \pm6.19\%$}} & \shortstack[r]{60.58\%\\ {$\scriptsize \pm6.78\%$}} & \shortstack[r]{47.12\%\\ {$\scriptsize \pm6.92\%$}} \\
\midrule

\multirow{2}{=}{\shortstack[l]{GPT}}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{22.12\%\\ {$\scriptsize \pm5.76\%$}} & \shortstack[r]{11.06\%\\ {$\scriptsize \pm4.35\%$}} & \shortstack[r]{5.29\%\\ {$\scriptsize \pm3.10\%$}} & \shortstack[r]{3.37\%\\ {$\scriptsize \pm2.50\%$}}
& \shortstack[r]{40.38\%\\ {$\scriptsize \pm6.80\%$}} & \shortstack[r]{23.08\%\\ {$\scriptsize \pm5.84\%$}} & \shortstack[r]{10.58\%\\ {$\scriptsize \pm4.27\%$}} & \shortstack[r]{6.25\%\\ {$\scriptsize \pm3.36\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{56.25\%\\ {$\scriptsize \pm6.88\%$}} & \shortstack[r]{51.44\%\\ {$\scriptsize \pm6.93\%$}} & \shortstack[r]{45.19\%\\ {$\scriptsize \pm6.90\%$}} & \shortstack[r]{38.94\%\\ {$\scriptsize \pm6.76\%$}}
& \shortstack[r]{100.00\%\\ {$\scriptsize \pm0.00\%$}} & \shortstack[r]{92.31\%\\ {$\scriptsize \pm3.69\%$}} & \shortstack[r]{82.69\%\\ {$\scriptsize \pm5.25\%$}} & \shortstack[r]{72.60\%\\ {$\scriptsize \pm6.19\%$}} \\

\addlinespace[2pt]
\multicolumn{10}{@{}l}{\textbf{Classifier: LlamaPG-2-FT-Cal30}} \\*
\midrule
\multirow{2}{=}{SA-WC-HC}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{88.76\%\\ {$\scriptsize \pm6.70\%$}} & \shortstack[r]{76.40\%\\ {$\scriptsize \pm9.00\%$}} & \shortstack[r]{76.40\%\\ {$\scriptsize \pm9.00\%$}} & \shortstack[r]{64.04\%\\ {$\scriptsize \pm10.17\%$}}
& \shortstack[r]{88.76\%\\ {$\scriptsize \pm6.70\%$}} & \shortstack[r]{76.40\%\\ {$\scriptsize \pm9.00\%$}} & \shortstack[r]{76.40\%\\ {$\scriptsize \pm9.00\%$}} & \shortstack[r]{64.04\%\\ {$\scriptsize \pm10.17\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{100.00\%\\ {$\scriptsize \pm0.00\%$}} & \shortstack[r]{100.00\%\\ {$\scriptsize \pm0.00\%$}} & \shortstack[r]{95.51\%\\ {$\scriptsize \pm4.39\%$}} & \shortstack[r]{95.51\%\\ {$\scriptsize \pm4.39\%$}}
& \shortstack[r]{100.00\%\\ {$\scriptsize \pm0.00\%$}} & \shortstack[r]{100.00\%\\ {$\scriptsize \pm0.00\%$}} & \shortstack[r]{95.51\%\\ {$\scriptsize \pm4.39\%$}} & \shortstack[r]{95.51\%\\ {$\scriptsize \pm4.39\%$}} \\
\midrule

\multirow{2}{=}{Gemini-HC}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{62.02\%\\ {$\scriptsize \pm6.73\%$}} & \shortstack[r]{38.94\%\\ {$\scriptsize \pm6.76\%$}} & \shortstack[r]{27.40\%\\ {$\scriptsize \pm6.19\%$}} & \shortstack[r]{16.35\%\\ {$\scriptsize \pm5.13\%$}}
& \shortstack[r]{62.50\%\\ {$\scriptsize \pm6.71\%$}} & \shortstack[r]{39.90\%\\ {$\scriptsize \pm6.79\%$}} & \shortstack[r]{27.40\%\\ {$\scriptsize \pm6.19\%$}} & \shortstack[r]{16.35\%\\ {$\scriptsize \pm5.13\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{96.63\%\\ {$\scriptsize \pm2.50\%$}} & \shortstack[r]{89.42\%\\ {$\scriptsize \pm4.27\%$}} & \shortstack[r]{79.81\%\\ {$\scriptsize \pm5.57\%$}} & \shortstack[r]{75.00\%\\ {$\scriptsize \pm6.00\%$}}
& \shortstack[r]{97.12\%\\ {$\scriptsize \pm2.32\%$}} & \shortstack[r]{89.90\%\\ {$\scriptsize \pm4.18\%$}} & \shortstack[r]{80.77\%\\ {$\scriptsize \pm5.47\%$}} & \shortstack[r]{75.48\%\\ {$\scriptsize \pm5.97\%$}} \\
\midrule

\multirow{2}{=}{GPT-HC}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{24.52\%\\ {$\scriptsize \pm5.97\%$}} & \shortstack[r]{14.42\%\\ {$\scriptsize \pm4.87\%$}} & \shortstack[r]{8.17\%\\ {$\scriptsize \pm3.80\%$}} & \shortstack[r]{5.29\%\\ {$\scriptsize \pm3.10\%$}}
& \shortstack[r]{43.27\%\\ {$\scriptsize \pm6.87\%$}} & \shortstack[r]{24.04\%\\ {$\scriptsize \pm5.93\%$}} & \shortstack[r]{12.50\%\\ {$\scriptsize \pm4.59\%$}} & \shortstack[r]{7.21\%\\ {$\scriptsize \pm3.59\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{62.98\%\\ {$\scriptsize \pm6.70\%$}} & \shortstack[r]{47.12\%\\ {$\scriptsize \pm6.92\%$}} & \shortstack[r]{39.90\%\\ {$\scriptsize \pm6.79\%$}} & \shortstack[r]{37.50\%\\ {$\scriptsize \pm6.71\%$}}
& \shortstack[r]{97.12\%\\ {$\scriptsize \pm2.32\%$}} & \shortstack[r]{78.37\%\\ {$\scriptsize \pm5.71\%$}} & \shortstack[r]{68.75\%\\ {$\scriptsize \pm6.43\%$}} & \shortstack[r]{62.98\%\\ {$\scriptsize \pm6.70\%$}} \\
\midrule

\multirow{2}{=}{\shortstack[l]{Gemini}}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{51.92\%\\ {$\scriptsize \pm6.93\%$}} & \shortstack[r]{35.10\%\\ {$\scriptsize \pm6.62\%$}} & \shortstack[r]{23.56\%\\ {$\scriptsize \pm5.88\%$}} & \shortstack[r]{14.42\%\\ {$\scriptsize \pm4.87\%$}}
& \shortstack[r]{64.90\%\\ {$\scriptsize \pm6.62\%$}} & \shortstack[r]{44.71\%\\ {$\scriptsize \pm6.89\%$}} & \shortstack[r]{30.77\%\\ {$\scriptsize \pm6.40\%$}} & \shortstack[r]{19.71\%\\ {$\scriptsize \pm5.52\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{73.08\%\\ {$\scriptsize \pm6.15\%$}} & \shortstack[r]{59.13\%\\ {$\scriptsize \pm6.82\%$}} & \shortstack[r]{48.08\%\\ {$\scriptsize \pm6.93\%$}} & \shortstack[r]{37.02\%\\ {$\scriptsize \pm6.70\%$}}
& \shortstack[r]{87.98\%\\ {$\scriptsize \pm4.51\%$}} & \shortstack[r]{72.60\%\\ {$\scriptsize \pm6.19\%$}} & \shortstack[r]{60.58\%\\ {$\scriptsize \pm6.78\%$}} & \shortstack[r]{47.12\%\\ {$\scriptsize \pm6.92\%$}} \\
\midrule

\multirow{2}{=}{\shortstack[l]{GPT}}
& \raisebox{3pt}{Conf-Guard}
& \shortstack[r]{22.60\%\\ {$\scriptsize \pm5.80\%$}} & \shortstack[r]{11.06\%\\ {$\scriptsize \pm4.35\%$}} & \shortstack[r]{5.77\%\\ {$\scriptsize \pm3.23\%$}} & \shortstack[r]{4.33\%\\ {$\scriptsize \pm2.82\%$}}
& \shortstack[r]{42.79\%\\ {$\scriptsize \pm6.86\%$}} & \shortstack[r]{23.08\%\\ {$\scriptsize \pm5.84\%$}} & \shortstack[r]{11.54\%\\ {$\scriptsize \pm4.43\%$}} & \shortstack[r]{8.17\%\\ {$\scriptsize \pm3.80\%$}} \\*
& \raisebox{3pt}{Baseline}
& \shortstack[r]{56.25\%\\ {$\scriptsize \pm6.88\%$}} & \shortstack[r]{51.44\%\\ {$\scriptsize \pm6.93\%$}} & \shortstack[r]{45.19\%\\ {$\scriptsize \pm6.90\%$}} & \shortstack[r]{38.94\%\\ {$\scriptsize \pm6.76\%$}}
& \shortstack[r]{100.00\%\\ {$\scriptsize \pm0.00\%$}} & \shortstack[r]{92.31\%\\ {$\scriptsize \pm3.69\%$}} & \shortstack[r]{82.69\%\\ {$\scriptsize \pm5.25\%$}} & \shortstack[r]{72.60\%\\ {$\scriptsize \pm6.19\%$}} \\

\end{longtable}
\endgroup

